An exploration of fetish social networks and communities

Online Social Networks (OSNs) provide a venue for virtual interactions and relationships between individuals. In some communities, OSNs also facilitate arranging online meetings and relationships. FetLife, the worlds largest anonymous social network for the BDSM, fetish and kink communities, provides a unique example of an OSN that serves as an interaction space, community organizing tool, and sexual market. In this paper, we present a first look at the characteristics of European members of Fetlife, comprising 504,416 individual nodes with 1,912,196 connections. We looked at user characteristics in terms of gender, sexual orientation, and preferred role. We further examined the topological and structural properties of groups, as well as the type of interactions and relations between their members. Our results suggest there are important differences between the FetLife community and conventional OSNs. The network can be characterised by complex gender based interactions both from a sexual market and platonic viewpoint which point to a truly fascinating social network.

==> 4measures.tex <==
\section{Network measures}
\label{sec:measures}

We use a number of graph theory measures for doing our comparison. We first present a range from basic measures and characteristics such as degree distributions, relationship reciprocity, power law exponent, clustering coefficient (measure of density of triangular ties between adjacent nodes).

We then look into more complex measures such as the average path length, joint degree distribution (JDD, a measure of connectivity of one's neighbours), and assortativity, which indicate the relations between the nodes on a local basis. We also explore the hierarchical structure of the network using k-cores and Kernel density estimation. We analyse the effects of these measures in the next section, while a complete explanation of the theoretical definitions and implications of these measures is available in~\cite{fay2010weighted} and~\cite{haddadi2008tuning}.


==> 5.2content.tex <==

\section{Content analysis}
\label{subsec:demo_anal}



An important feature of the fetish network are fetish tags. Users chose free tags to label themselves or reuse existing tags which they see on other profiles or on a list of most frequent tags. 
In contrast to the user roles examined in the demographic analysis in section \ref{subsec:demo_anal}, the tags are chosen by the users themselves and allow us to gain objective insights in the subcommunities of the fetish network by detecting groups of users with similar tags. To the best of our knowledge, there exists no objective grouping of fetishes in literature. 
Using the self-descriptive tags from the fetish community, we are able to create a first objective, data based grouping of fetishes.


\newcolumntype{L}[1]{>{\hsize=#1\hsize\raggedright\arraybackslash}X}%
\newcolumntype{R}[1]{>{\hsize=#1\hsize\raggedleft\arraybackslash}X}%
\newcolumntype{C}[2]{>{\hsize=#1\hsize\columncolor{#2}\centering\arraybackslash}X}%

\begin{table*}[t]
\begin{minipage}[t]{0.76\textwidth}
\footnotesize{
\begin{tabularx}{1.3\textwidth}{ L{0.1} | L{1} | L{1} | L{1} | L{1} | L{1} | L{1} }
&
\multicolumn{1}{c|}{\textbf{\ Topic 1\ }}&
\multicolumn{1}{c|}{\textbf{\ Topic 2\ }}&
\multicolumn{1}{c|}{\textbf{\ Topic 3\ }}&
\multicolumn{1}{c|}{\textbf{\ Topic 4\ }}&
\multicolumn{1}{c|}{\textbf{\ Topic 5\ }}&
\multicolumn{1}{c}{\textbf{\ Topic 6\ }}
\\
\hline \hline 
\parbox[t]{0.8mm}{\multirow{20}{*}{\rotatebox[origin=c]{90}{Top 20 Tags by Probability}}}
&oral sex		&bondage		&bondage 			&watersports	&hair pulling			&latex\\
&rough sex		&oral sex		&discipline 		&rimming		&biting					&rubber\\
&blow jobs		&spanking		&humiliation 		&face sitting$^3$	&intelligence		&diapers		\\
&anal sex		&anal sex		&caning 			&golden showers	&princess$^1$			&bondage		\\
&hair pulling	&blindfolds		&spanking			&humiliation	&spanking$^4$			&cross dressing	\\
&kissing		&discipline		&orgasm control 	&ass worship	&spanking$^2$			&leather		\\
&deep throating	&handcuffs		&pain				&mistresses$^5$	&respect				&catsuits 		\\
&lingerie 		&master/slave	&collar$^6$ 		&	femdom 		&spanking 				&corsets \\
&talking dirty 	&whips 			&breast torture$^7$ &		strap-ons &		cuddles 	&ball gags \\
&spanking 		&dildos 		&obedience$^8$&		foot worship &		rough sex	&feminization\\
&bondage &		ass play &		bdsm &		anal stretching &		kissing &		pvc \\ 
&biting &		toys &		ball gags &		anal training &		pushed wall$^9$ &		high heels \\ 
&threesomes &		collar$^6$ &		face slapping &		anal sex &		face slapping &		masks \\ 
&cunnilingus &		breast torture$^7$ &		flogging &		ass to mouth &		throat$^{10}$ &		gas masks \\ 
&blindfolds &		humiliation &		candle wax &		face fucking &		lust &		vacuum bed \\ 
&photography$^{12}$ &		lingerie &		breath play &		foot/feet &		play rape &		mummification \\ 
&bare spanking$^{13}$ &		high heels &		whips &		ass play &		more complex$^{11}$ &		age play \\ 
&corsets &		candle wax &		domination &		humiliation$^{14}$ &		converse$^{15}$ &		costumes$^{16}$ \\ 
&intelligence &		pain &		bare spanking$^{13}$ &		fisting &		*me*$^{17}$ &		chastity devices \\ 
&masturbation &		masturbation &		caging$^{18}$ &		human toilet &		breath play &		diaper \\ 
\end{tabularx}
}
\end{minipage}
%\begin{minipage}{0.223\textwidth}
%
%\center
%
%\begin{scriptsize}
%\begin{spacing}{1.40}
%\textbf{Maps for Topic 1}
%\end{spacing}
%\end{scriptsize}
%\includegraphics[width=1\textwidth,natwidth=873,natheight=434]{img/map/foodMap2L.png}
%
%\vspace{0.01cm}
%
%\includegraphics[width=1\textwidth,natwidth=873,natheight=434]{img/map/foodMap2M.png}
%\end{minipage}
\\
\textit{
$^1$being treated like a beautiful princess but fucked like a dirty little whore
$^2$"the look" that tells you in no uncertain terms that you have crossed the line and earned a spanking
$^3$face sitting/smothering
$^4$bare handed spanking
$^5$mistresses with strap-ons
$^6$collar and lead/leash
$^7$breast/nipple torture
$^8$obedience training
$^9$being pushed up against a wall in a passionate kiss
$^{10}$being fucked with a hand on my throat and threats being whispered into my ear
$^{11}$being more complex than an anonymous list of fetishes could show
$^{12}$erotic photography
$^{13}$bare bottom spanking
$^{14}$verbal humiliation and degradation
$^{15}$causing people to have to actually converse with me
$^{16}$costumes/dressing-up
$^{17}$finding out if they like *me* and not just what gets me off.
$^{18}$caging/confinement
}
\caption{
Topics extracted from user tags ordered by popularity. The twenty most probable words of each topic are shown.
}
\label{tab:fetishtopics}
\end{table*}

\subsection{Detection of Fetish Topics}

For the tag-based grouping of users we rely on techniques from probabilistic topic modelling developed for text analysis. 
Topic models allow us to detect latent factors that explain the co-occurrence of terms in documents. \cite{blei2003latent}

In order to clean the data, we remove words tags which appear less than ten times in the dataset.
Users can classify their tags as fetishes they are practising and fetishes they are interested in. They also can specify if they are the giving or receiving part of a practice. For increasing the evidence for learning the probabilistic model, we ignore such additional information and focus on the sexual practices.

We use data from Europe for detecting the fetish topics. As we expected to see regional variation in the fetishes, we learned a geographical topic model for capturing those differences. The geographic location of a user is given in the user profile as a city (in Great Britain) or an administrative region (for the rest of Europe).
We chose a Multi-Dirichlet based topic model (MGTM) by Kling et al. \cite{kling:mgtm} to model the data as the model is non-parameteric, e.g. the number of topics is learned by the model during inference. Therefore the resulting topics are the objective statistical description of the data which explains the observed patterns best.
The topics detected are shown in Table \ref{tab:fetishtopics}.

It is possible to interpret probabilistic topics based on the top words\cite{blei2003latent}. We interpret our topics based on the top-20 words as follows:
\textbf{Topic~1} represents rough oral sex. 
\textbf{Topic~2} is very similar but more focussed on sado-masochistic (SM) practices. 
\textbf{Topic~3} then represents harder SM sex. 
\textbf{Topic~4} is focussed on excrements and ''dirty'' practices. 
\textbf{Topic~5} is centred around rough sex but also includes the fetish for intelligence, respect and cuddling - an ambivalent motif. 
Finally, \textbf{Topic~6} is about clothing and accessories - all top tags are materials or objects worn on the skin.


\subsection{Regional and Demographic Patterns}

Surprisingly, we found no geographical patterns of the topics, except for isolated outliers in single locations. Topic probabilities vary less than 1\% within whole Europe. This indicates that the topics behind sexual fetishes are universal within the community and are stable across cultures.

We then tested for deviations of topic occurrences within groups of different age, gender, sexual orientation and relationship status.
To our great surprise, there are no significant differences in the rate of occurrence for all six topics.
In order to check these findings, we looked at the frequency of single tags for different groups of users.
Here we found bigger deviations, e.g. for the term lingerie which is more popular with transvestites (0.26\%) than with men (0.15\%). 
However, the overall frequency of the top terms of Topic 6 in total is nearly identical for both groups.
This observation was repeated for all groups.

This finding indicates that the latent motives behind the choice of fetishes are shared among all members of the network.
It is the socio-cultural context such as gender, age or orientation which then determines how the motif is lived out as sexual behaviour.

